ChameleonControl: Teleoperating Real Human Surrogates through Mixed Reality Gestural Guidance for Remote Hands-on Classrooms

We present ChameleonControl, a real-human teleoperation system for scalable remote instruction in hands-on classrooms. In contrast to existing video or AR/VR-based remote hands-on education, ChameleonControl uses a real human as a surrogate of a remote instructor. Building on existing human-based telepresence approaches, we contribute a novel method to teleoperate a human surrogate through synchronized mixed reality hand gestural navigation and verbal communication. By overlaying the remote instructor's virtual hands in the local user's MR view, the remote instructor can guide and control the local user as if they were physically present. This allows the local user/surrogate to synchronize their hand movements and gestures with the remote instructor, effectively teleoperating a real human. We deploy and evaluate our system in classrooms of physiotherapy training, as well as other application domains such as mechanical assembly, sign language and cooking lessons. The study results confirm that our approach can increase engagement and the sense of co-presence, showing potential for the future of remote hands-on classrooms.

==> feedback.tex <==

\subsection{The First User Study}

Other comments:
\textit{``P20: VR technology is not fully mature, it still has a gap between it and real class.''}
\textit{``P4: I believe it is either zoom or fake see through glass makes this more better than other options.''}
\textit{``P4: I believe it is either zoom or fake see through glass makes this more better than other options.''}
\textit{``P3: The zoom presentation to me was the worse because even though it has its benefit it is more difficult because it just seems like a live pre recorder video''}
P15: I like seeing in person
For the zoom lesson and virtual hands it feels like your watching a video
\textit{P19: Not being able to see a demonstration from the virtual hands, I’m not fully able to tell what presence I feel from it''}
\textit{``P4: We can connect more with the instructor live''}
but having the face on the IPad didn’t make any difference for me

I liked how everything was in VR or zoom I feel like lots of people would learn more even if there not there because let's say there sick and can't be somewhere in person they would have this to still learn
I liked the fact that you could see the persons face demonstrating the instructors action most in the real person with fake see through AR headset
I put lower grades for all, because I think the real engagement would be with real person
Each method I feel makes it harder to learn accurately
Seeing the massage in person is something I find easier to understand




\subsection{The Second User Study}

OTHER COMMENTS:
\textit{``P3: Heared instructions clearly''}
\textit{``P7: Inmersive it's easy to use''}
\textit{``P9: It's better''}
\textit{``P10: AR-because you can do it together with your instructor. 1st zoom- not as much as VR. 3rd zoom- not as much as VR''}
\textit{``P11: I found the car hand extremely hard to follow, I enjoyed the experience though''}
\textit{``P12: The numbers I chose are based on how well I felt when following the instructions.''}
\textit{``P1: Seeing the hands on the client with mine helps me understand pace and where to be better''}
\textit{``P3: Easy to hear''}
\textit{``P5: immersive and 1st person were both easy to understand. 3rd person again couldn't see as much''}
\textit{``P6: Same answer as above''}
\textit{``P7: Easy to use''}
\textit{``P9: I understand the instructor well''}
\textit{``P10: VR- because you can do it with your instructor by seeing his/her hand. 1st- not as much as VR. 3rd-not as much as VR.''}
\textit{``P12: Again, it is based on how well I could follow instructions''}
\textit{``P1: Ar felt best. The help was right onto of my hands.''}
\textit{``P2: AR- very engaging almost like a video game. It was a different feel and it kept my attention. 1st- I was engaged to a certain extent it felt more like just watching a regular video. 3rd. Almost the same as 1st. It did give me a chance to practice body mechanics''}
\textit{``P3: Good experience''}
\textit{``P4: I felt the same amount of engagement for them all''}
\textit{``P5: immersive was really engaging because of the hand tracing 1st and 3rd person was just demonstrating''}
\textit{``P6: Same answer as above''}
\textit{``P7: The AR lessons easy to use and understand''}
\textit{``P8: All your senses are engaged at once''}
\textit{``P9: The instructor deliver the instruction well and can follow easily''}
\textit{``P10: VR- because you can do it with your instructor by seeing his/her hand. 1st- not as much as VR. 3rd-not as much as VR.''}
\textit{``P11: I really felt that the Vr experience was the most engaging''}
\textit{``P12: Mostly based on the advice or what the instructor have said.''}

\textit{``P2: 3rd- following was east as well and I especially appreciate the view of body mechanics''}
\textit{``P2: 3rd was great for body mechanic''}
CO-PRESENCE
\textit{``P2: The 1st person video gave more of a reality you could tell how much pressure to apply.''}
3rd person feels impersonal. I can't see properly what the teacher is doing. 
INFORMATIVE
\textit{``P1: Fairly clear. Bit with the ghost hands we can be sure.''}
\textit{``P2: For each video it was very informative. I was able to follow along. Again just the lack of reality with AR in that I wasn’t able to follow pressure or body mechanics wise. Everything else was good.''}
\textit{``P3: Should have video game suit to be accurate''}
\textit{``P4: The hands were hard to make out most of the time but the voice helped in ar, in the videos it's clear what he is doing and how it should be done''}
\textit{``P5: immersive and 1st person was clear to understand and 3rd person I couldn't see as much''}
\textit{``P6: Same answer as above''}
\textit{``P7: feel that we are in person''}
\textit{``P8: You can't miss the information provided''}
\textit{``P9: It's clear and can follow easily to the instructor''}
\textit{``P10: VR- because you can do it with your instructor by seeing his/her hand. 1st- not as much as VR. 3rd-not as much as VR''}
\textit{``P11: Again just struggled keeping my hands on the instructions hands''}
\textit{``P12: Mostly based on the engagement and advice the instructor gave.''}
\textit{``P11: The instructor was still able to help me, but it was nothing like having them in class with you''}



==> rebuttal.tex <==
We thank the reviewers for their insights and helpful comments. We outline how we will address these to improve the paper:

=== REBUTTAL === 

First, we would like to clarify that the originality and significance of our contribution lies in our idea of "real-human teleoperation" and "repurposing" of a local surrogate as a classroom instructor". Our work differs from other research in the field, such as Huang's (R3), which only explored and evaluated one-on-one settings without having a student audience and/or without focusing on synchronization of human motion.

Our overall contribution is not a single study, but includes the combination of the concept, design goals, system, and evaluations. Our final study is just one part of it. We argue that it is not appropriate to solely evaluate our contribution based on the resemblance of the final study to other work. Moreover, the goal of our final study was to explore the generalizability of our idea and gain a better understanding of promising and non-promising tasks. The evaluation criteria we used was the accuracy of behavior synchronization, which is different from the common goal of remote collaboration, such as Huang's (R3), where the focus is on effective communication.

The first study does not debunk our motivation. The two ChameleonControl interfaces (with/without face) provide insights on whether the presence or absence of a 2D face affects our goal of remotely teleoperating humans for scalable classroom education. From the system's implementation point of view, yes, it seems similar to the prior work, but the goal and purpose is completely different and unique. In both conditions, the local students can still see the remote expert's "physical demonstration", regardless of whether the face is present. Therefore, we do not think this contradicts to the original motivation and background. And again, the 2D face is simply one part of the condition, and we argue that it is not appropriate to solely evaluate our contribution based on it. 


SYSTEM CONCEPT AND DESIGN [R1, R3]

R1 requested clarification on users resolving ambiguity in hand gestures. We agree with the feedback and have elaborated on the methods with which surrogate’s communicate with remote users. Specifically, we did not mention in our previous submission that surrogates and remote users can communicate verbally via an internet call, either through the iPad face or a separate device when the iPad face wasn’t used.

We agree with R2 that simply stating that surrogates are usually students in the System and Implementation section is confusing and unclear. We expand and elaborate on this. Specifically, we explain the requirements to act as a surrogate are the ability to properly replicate the remote instructors’ instructions/demonstration/lesson. We explain that depending on the use case, there could be different requirements. For example, surrogates could be seated for certain lessons or only require the use of one hand, etc. We then explain that we envision surrogates to usually be students or teaching assistants in the context of remote instruction for hands-on classrooms.

R3 requested clarification regarding where some design decisions are derived from. Specifically, R3 believed that some expert interviewees provided guidance outside of their expertise. We hope to make our system implementation and formative study clearer by swapping sections 3.2 and 3.3 so that the system implementation follows the formative study instead of vice-versa. Additionally, we clarify and rephrase the 4th design goal to be closer to what our experts had actually said rather than how we interpreted it.


UNCLARITIES IN PRESENTATION [R2, R3]

We agree with the reviewers that the abstract doesn’t fully reflect the paper, it’s findings or it’s structure. We have rewritten the abstract to better reflect our novelty, contribution, findings and the overall paper structure.

We agree with the reviewers that our figures require clarification, particularly the graphs as they were illegible without any legend to distinguish the results. We have totally overhauled the figures and made them significantly easier to understand.

We agree with R3 that we should include details on how our questionnaire was developed. To this end, we've included an explanation of what questions we asked and the prior research and relevant works that our questionnaire was inspired by and partially derived from.

MISSING DISCUSSION [R2]

We agree with the reviewers that our paper can be improved with an additional discussion on the ethics of using human surrogates. We’ve done so, clarifying that our system can only enable ethical use of human surrogates but exploring hypothetical unethical uses. For example, we discuss the potential for dehumanization of surrogates, particularly when their human characteristics (face, body, voice, etc) are replaced with another person's. Additionally, we discuss the potential for in-voluntary synchronization using technologies like Electro-Muscle Stimulation (EMG). We explain that such technologies could enable malicious or accidental synchronization between users, forcing surrogates to perform acts against their will.

We agree with the reviewers that discussion of “the uncanny valley” is relevant. We elaborate on this in our discussion of why students preferred a see-through mixed reality headset such as the Hololens. We explain that one possible reason for this could be that, because the 2D iPad face poorly replicates the remote instructor's face , it therefore invokes an uncanny valley effect in the student audience who perceive it as "off-putting" and "creepy". This could provide further insight into why see-through mixed reality headsets were most requested by students. We also elaborate on the practical issues with using a 2D display to replace a surrogate’s face with a remote instructor’s. 

We agree with the reviewers that a discussion of the ethics of using human surrogates is warranted. We elaborate on our system's limitation in that it can only enable “voluntary” synchronization. We also hypothesize potential unethical uses of human surrogates, such as by forcing synchronization of a user with another via electro-muscular stimulation (EMGs) ex: by using a TeslaSuit to force a user to perform acts/behaviors against their will. This kind of “involuntary” synchronization could occur mistakenly or maliciously by a remote user. Additionally, we discuss the potential for dehumanization of human surrogates by replacing their body, behavior and actions with those of a remote user. Careful consideration should be taken for the wellbeing of human surrogate.



















=== CHANGE LOG === 
Below, we describe how we addressed the concerns. 

- Missing detail on how questionnaire is developed [R3]
Added the actual questionnare in 4.2.3
These questions are partially derived from the literature
e.g., co-presence: [ 1, 44 , 50 ], engagement: [ 1 ], easy
to understand: [50, 66], etc) 

- Design goals [R3]
we swapped 3.2 and 3.3.
we also rephrased the fourth design goals to be closer to what they actually mentioned, rather than how we interpreted 

- Abstract [R2] 
Fixed 
Fixed intro too

- Figures [R2, R3]
Fixed Figure 2 and 3. 
Added some additional figures

- Discussion (uncanny valley) [R2]
Added in Discussion Section

- Discussion (ethics) [R2]
Added in Discussion SectionAdded 

- Discussion (ambiguity) [R1]
Added in Discussion Section
Explain a bit more

- At the end of page 5, the authors claim, “The local surrogate is usually a student…”. I understand that this information might have originated from the formative study. However, at this time of the manuscript, it is hard to tell why surrogates are students. [R2] 
[Mehrad] - Done

- Statistical analysis [R3]
we did. we only found [x] for the statistical significance. 


% - The originality and significance could be clearer, as the work is not sufficiently contrasted to expert-worker remote guidance in XR literature, e.g., Huang’s work (R3).
% - There is a mismatch between the background literature motivating the idea and the insignificant results of the first study (R3)

% > This is an issue, as the underlying background does not go into much detail in how the underlying system is an improvement on the state of the art when you remove the attached tablet display.



% - Augmented Studio
% - Evaluating the Combination of Visual (Co-presence)
% - Integrating AR/MR/DR technology in remote seal to maintain confidentiality information (easy to understand)
% - Mixed Reality Remote Collaboration Combining 360Video and 3D Reconstruction (understand, co-presence, 
% - Wearing Another’s Personality:
% - MeBot (engaging, co-presence)



% First of all, we would like to clarify that the originality and significance of the contributions come from  1) the idea of "real-human teleoperation" and 2) the repurpose of the local surrogate as a classroom instructor. 

% > expert-worker remote guidance in XR literature, e.g., Huang’s work (R3)

% Huang's work does not explore either of 1 and 2 directions. Their work, including others, only explored and evaluated for one-on-one settings. More specifically, they did not use the remote guidance for student audience, and they did not use it for synchronizing the human motion, as opposed to remote "guidance". 

% > the final studies are indeed a direct evaluation of hand gesture direction in an XR environment.

% First of all, the final study is just a part of the entire contributions (concept, design goals, system, evaluations). It is not appropriate to solely evaluate the contribution solely because of the resemblance of the final study. 
% Second, the goal of the final study is the exploration of the generalizability of the idea and have a better understanding what tasks would be promising and what are not. 
% Third, the evaluation criteria is how acruately the behavior can be synchronized, which is different from the common goal of the remote collaboration where they are interested in how effective it can communicates for collaboration (communication vs synchronization). 

% > The first study however debunks this notion, with no differences in the two ChameleonControl interfaces (with/without face). 

% First, again, this two conditions are just a part of the entire contribution. 
% Second, we do not think this debunks our motivation. 
% Our goal has been how to remotely teleoperate humans for scalable classroom education. The condition of whether it has a face or not does not entirely affect this goal. 
% The local students can still see the remote expert's "physical demonstration". The face is again just a part of the condition. 




